YuriiFormer: A Suite of Nesterov-Accelerated Transformers

We propose a variational framework that interprets transformer layers as iterations of an optimization algorithm acting on token embeddings. In this view, self-attention implements a gradient step of an interaction energy, while MLP layers correspond to gradient updates of a potential energy. Standard GPT-style transformers emerge as vanilla gradient descent on the resulting composite objective, implemented via Lie--Trotter splitting between these two energy functionals. This perspective enables principled architectural design using classical optimization ideas. As a proof of concept, we introduce a Nesterov-style accelerated transformer that preserves the same attention and MLP oracles. The resulting architecture consistently outperforms a nanoGPT baseline on TinyStories and OpenWebText, demonstrating that optimization-theoretic insights can translate into practical gains.

==> tikz/arch_common_styles_aiayn.tex <==
% Common TikZ styles for architecture diagrams, inspired by
% "Attention Is All You Need" (Vaswani et al., 2017).
%
% Use from standalone figures via: \input{arch_common_styles_aiayn.tex}
\usepackage{amsmath,amssymb}
\usepackage{xcolor}

\usetikzlibrary{positioning,arrows.meta,calc}

% Pastel palette (approx. from the paper diagrams)
\definecolor{aiaynBlue}{HTML}{CFE8F8}
\definecolor{aiaynOrange}{HTML}{FAD7A0}
\definecolor{aiaynYellow}{HTML}{F9E79F}

\tikzset{
  block/.style={
    rectangle,
    draw=black,
    line width=0.9pt,
    rounded corners=2pt,
    align=center,
    inner sep=4pt,
    minimum height=0.95cm,
    minimum width=1.45cm,
    font=\sffamily\small
  },
  ln/.style={
    block,
    fill=aiaynYellow,
    minimum width=1.00cm
  },
  attn/.style={
    block,
    fill=aiaynOrange
  },
  mlp/.style={
    block,
    fill=aiaynBlue
  },
  addop/.style={
    circle,
    draw=black,
    line width=0.9pt,
    minimum size=0.65cm,
    inner sep=0pt,
    font=\sffamily\small
  },
  state/.style={font=\normalsize},
  arr/.style={-{Latex[length=2.0mm,width=2.0mm]}, draw=black, line width=0.9pt},
  skip/.style={arr, rounded corners=6pt}
}


